Batch Multi-Fidelity Bayesian Optimization with Deep Auto-Regressive Networks

Bayesian optimization (BO) is a powerful approach for optimizing black-box, expensive-to-evaluate functions. To enable a flexible trade-off between the cost and accuracy, many applications allow the function to be evaluated at different fidelities. In order to reduce the optimization cost while maximizing the benefit-cost ratio, in this paper, we propose Batch Multi-fidelity Bayesian Optimization with Deep Auto-Regressive Networks (BMBO-DARN). We use a set of Bayesian neural networks to construct a fully auto-regressive model, which is expressive enough to capture strong yet complex relationships across all the fidelities, so as to improve the surrogate learning and optimization performance. Furthermore, to enhance the quality and diversity of queries, we develop a simple yet efficient batch querying method, without any combinatorial search over the fidelities. We propose a batch acquisition function based on Max-value Entropy Search (MES) principle, which penalizes highly correlated queries and encourages diversity. We use posterior samples and moment matching to fulfill efficient computation of the acquisition function and conduct alternating optimization over every fidelity-input pair, which guarantees an improvement at each step. We demonstrate the advantage of our approach on four real-world hyperparameter optimization applications.

==> exp.tex <==
\section{Experiment}
%\vspace{-0.1in}
\subsection{Synthetic Data}

We first evaluate the prediction accuracies of different multi-fidelity surrogate modelings on two synthetic functions: \textit{Branin} and \textit{Levy}. Our multi-fidelity formulations of those two functions can be found in the supplementary materials. Prediction accuracy is critical for Bayesian Optimization. We compared our full autoregressive models with Hamiltonian Monte-Carlo sampling with following baselines: sequential autoregressive deep neural nets with variational posterior(DNN-MFBO), multi-fidelity Gaussian process which fidelities are correlated with Gaussian Process errors(MF-MES), and multi-task Gaussian Process, which assumes independent Gaussian process for each fidelity with bounded errors(MF-GP-UCB). 

The sequential and full autoregressive surrogate models are neural networks based. For each fidelity, we use two hidden layers with 40 neurons and choose tanh as the activation function. For the full autoregressive models, we use the Hamiltonian Monte-Carlo sampler implemented by (https://github.com/AdamCobb/hamiltorch). We set the HMC sampler by burning 5000 samples and sample 200 posterior samples every 10 steps. And for the multi-fidelity and multi-task GP methods, we used RBF kernels. 

We iteratively evaluate prediction accuracy like the Bayesian Optimization. We first prepare an initial training set with a small number of samples. At each iteration, we append the training set with additional training examples by uniformly sampling from the input space. We initialize the training set size as 10 for the first fidelity and 5 for the second fidelity for two-fidelities Levy. We add an additional 5 examples of the first fidelity and 1 example of the second fidelity to the training set at each iteration. For three-fidelities Branin, we initialize the training set size as 20 for the first fidelity, 10 for the second fidelity, and 5 for the highest fidelity. We add 5, 2, 1 examples to the training set at each iteration. The prediction accuracies are evaluated on a separate multi-fidelity testing set acquired by uniformly sample from the input space then query the ground truth from the synthetic functions. We prepare 100 testing examples for each fidelity. The plot(add later) shows the prediction normalized root mean squared error (nRmse) along with the number of iterations.

\subsection{Real-World Applications}

Secondly, we test our proposed methods on several well-known domains, including Latent Dirichlet Allocation, XGBoost, Convolutional Neural Networks, and Physical-Informed Neural Networks. All of the domains are known to be sensitive to the hyper-parameters settings and require their users spend a lot of time tuning their performance on specific tasks. We compared proposed methods with several state-of-art single fidelity, multi-fidelity Bayesian optimization/hyperparameter optimization tools. Include,
\begin{itemize}
	\item MF-GP-UCB
	\item MF-MES
	\item Scalable Hyperparameter Transfer Learning (HPO)
	\item SMAC
	\item Parallel-MF-MES
	\item GP-Kernel
	\item GP-Thompson Sampling
\end{itemize}
Our proposed methods include:
\begin{itemize}
	\item Single Query 
	\item Parallel Batch Query
	\item Info-Gain Greedy Batch Query
	\item  Bounded Info-Gain Batch Query
\end{itemize}
In addition to justify the performace of methods, we also compare the fully random-strategy which at each hyperparameter optimize iteration, we randomly choose a fidelity level and an input for query. The metric of evaluating the performance of the hyperparameter tuning and the definition of fidelity in multi-fidelity tunning varies from the domains. Now, we are going to describe the details.

As in the synthetic experiment settings, for the neural network-based methods, we set hidden layers width to 40 and the hidden layers depth to 2 and use tanh as the activation function. For GP based methods, we used RBF kernels. Note that the Scalable Hyperparameters transfer learning does not have a cascade structure; we use the same setting for the features network and then set the features dimension to 32. We run each compared method 5 times and report the tuning performace with mean and standard deviation along with the total costs.

\subsubsection{Online Latent Dirichlet Allocation}

The first domain we are interested in is tunning the performance of the online variational Bayes algorithm for Latent Dirichlet Allocation. Unlike conventional or full batch LDA, online LDA uses stochastic optimization with natural gradient steps, which converges to the local minimum of the Variational Bayes objective. Online LDA is known to handle massive document collection in a streaming way. However, several hyperparameters need to be appropriately set to ensure the online LDA produces good results. We conduct seven tunable hyperparameters of the online LDA model: document topic prior (alpha in the original online LDA paper), which is continuous takes the value from [1e-3, 1.0], topic word prior(eta in the paper), which is continuous takes the value from [1e-3, 1.0], learning decay which is the learning rate takes from [0.51, 1.0], stopping tolerance for updating a document in E-step takes the range [1e-5, 1e-1], learning offset which is a positive parameter that down weights early batches in the online setting takes value from [1.1, 2.0, 5.0, 10.0, 20.0, 50, 100, 200], the batch size take from [2,4,8,16,32,64,128,256] and the number of topics K takes the value from [1, 64]. We encode the categorical and discrete hyperparameters into their binary encodings. So the space of hyperparameters has a dimension of 16 for online LDA.  We test the online LDA performance on the 20 Newsgroups dataset, which has over 18000 documents. We isolate 5000 documents for training the online LDA model then test the perplexity on another set of 1000 documents.

We formulate the multi-fidelity setting of online LDA as the maximum iterations could take in the training procedure. In our experiment, we use three fidelity levels. For the low-fidelity, we set the maximum iterations to 1. For the medium-fidelity, we set the maximum iterations to 10, and for the high-fidelity, we set the maximum iterations to 50. To properly initialize the surrogate model for hyperparameter optimization, we prepare a multi-fidelity initial dataset where the inputs are uniformly sampled from the encoded hyperparameters space. The outputs are acquired by training the online LDA model and test the perplexities.  We prepared 10 training examples for each fidelity. We used the same initialization dataset for each compared method.

\subsubsection{XGBoost Regreesor}

Gradient boosting is a generalization of boosting to arbitrary differentiable loss functions. Gradient boosting is effective that can be applied to both regression and classification problems. For the Gradient boosting, we introduce 7 hyperparameters for tuning: alpha in the Huber loss ranges from [0.01~0.1], the non-negative complexity parameter used for minimal cost-complexity pruning ranges from [0.01, 100], the fraction of samples to be used for fitting the individual base learners ranges from [0.1~1.0], the fraction of number of features to consider when looking for the best split ranges from [0.01, 1.0], criteria used for splitting chosen from MAE criteria or MSE criteria, the minimum number of samples required to split an internal node ranges from [2-9], and the maximum depth of individual regression learner ranges from [1,16]. We also encode the categorical and discrete variables into their binary encodings. So the total input dimension of hyperparameter searching is 12. We tune the performance of gradient boosting on the diabetes dataset. The diabetes dataset has 442 examples in total, and we use two-third of the dataset for training and one-third for testing the gradient boosting prediction accuracy in terms of the normalized root mean squared errors(nRmse).

We formulate the context of multi-fidelity learning of gradient boosting in terms of how many weak learners are used. In our experiment, the low-fidelity boosting algorithm uses 2 weak learners; the middle-fidelity algorithm uses 10 weak learners, and high-fidelity uses 100 weak learners. For the diabetes dataset, 100 learners are sufficient to achieve good performance. We also prepare 10 training examples of each fidelity to initialize the hyperparameters tuning algorithms for each compared method.

\subsubsection{Convolutional Neural Network}

A convolutional neural network is a deep learning model that takes images and input, assigns learnable weights and biases to various aspects/objects in the images. It can capture spatial dependencies in an image by introducing relevant filters and has achieved great success in the computer vision community. The network can be trained to understand the sophistication of an image better. ConvNet, in general, is a wealthy family in representation. It is known to be sensitive to the structure chosen and requires an experienced user to spend the effort searching in hyperparameters space. Traditional searching strategies include grid search, and random search might work for small scale network structure and dataset. However, when the model itself requires extensive training, those two simple strategies will still fail if the budget is limited. 

In our experiment, we formulate our hyperparameters tuning space as follows: the number of convolutional layers ranges from [1,4], the number of first convolutional filter's channels ranges from [8, 136], the hidden depth of fully connected layers ranges from [1,8], the hidden width of the fully connected layers ranges from [32,2080], the pooling type choose from ['max-pooling,' 'average pooling'] and the dropout rate ranges from [1e-3, 0.99]. We still applied binary encoding for categorical and discrete variables, the dimension of the hyperparameters tuning space is 25. Even with this restriction, the hyperparameters tuning space is still as rich as 17M possible combinations in categorical and discrete variables and continuous variables. It still forbids human researchers from searching exhaustively or using simple searching strategies. 

We use the CIFAR10 dataset to test the performance of the convolutional neural network. We prepare 10000 images for training and 10000 images for testing. We fix the mini-batch size to 100. The multi-fidelity setting in this problem is formulated as the number of epochs. We fixed the low-fidelity evaluation uses only one epoch training, middle fidelity uses 10 epochs training, and high-fidelity uses 50 epochs for training. The performance is evaluated as log-loss.

\subsubsection{Physics-informed Neural Networks}

The Physics-Informed Neural Networks(PINN) is a deep model that is trained to solve supervised learning problems where any general nonlinear partial differential equations give the data by the law of physics. These neural networks can infer the solutions of partial differential equations and obtain physics-informed surrogate models. The representation of PINN lies in fully connected neural networks, and it is known to be sensitive to the underlying FCNN structure and activation function. So in the PINN tuning task, our hyperparameters tuning space includes: the depth of the hidden layers ranges from [1,8], the width of hidden layers ranges from [1,64], and we select 8 different activation functions to include relu, tanh, sigmoid and their variations, etc. 

The dataset used for evaluating the performance PINN are solutions by numerical solvers of the Burgers equation. We set the viscosity as a small number where the Burgers has steep shoulders and is challenging to learn by the surrogate model. The PINN uses LBFGS as the optimizer inside its training procedure. So our multi-fidelity setting for tuning the hyperparameters of PINN is formulated as the maximum number of iterations in the LBFGS optimizer. Our low-fidelity evaluation set the maximum iterations to 10, and middle fidelity uses 100, and high-fidelity uses 50000 to encourage the convergence. And as in the previous experiment, we also prepare 10 evaluation results at each fidelity to initialize the hyperparameters tuning algorithms and use them across all the compared methods.

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/Diabetes_legend.eps}
	\vspace{-0.3in}
	%\vspace{-0.3in}
\end{figure}

\begin{figure}
%\vspace{-0.15in}
\centering
%\setlength\tabcolsep{0.01pt}
\includegraphics[width=0.48\textwidth]{./figs/Cifar10_legend.eps}
\vspace{-0.3in}
%\vspace{-0.3in}
\end{figure}

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/BurgersShock_legend.eps}
	\vspace{-0.3in}
	%\vspace{-0.3in}
\end{figure}

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/NewsGroup_legend.eps}
	\vspace{-0.3in}
	%\vspace{-0.3in}
\end{figure}

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/Branin_legend.eps}
	\vspace{-0.3in}
	%\vspace{-0.3in}
\end{figure}

\begin{figure}
	%\vspace{-0.15in}
	\centering
	%\setlength\tabcolsep{0.01pt}
	\includegraphics[width=0.48\textwidth]{./figs/Levy_legend.eps}
	\vspace{-0.3in}
	%\vspace{-0.3in}
\end{figure}


